UNcommonsense Reasoning: Abductive Reasoning about Uncommon Situations

Language technologies that accurately model the dynamics of events must perform commonsense reasoning. Existing work evaluating commonsense reasoning focuses on making inferences about common, everyday situations. To instead investigate the ability to model unusual, unexpected, and unlikely situations, we explore the task of uncommonsense abductive reasoning. Given a piece of context with an unexpected outcome, this task requires reasoning abductively to generate an explanation that makes the unexpected outcome more likely in the context. To this end, we curate and release a new English language corpus called UNcommonsense. We characterize the performance differences between human explainers and the best-performing large language models, finding that model-enhanced human-written explanations achieve the highest quality by trading off between specificity and diversity. Finally, we experiment with several imitation learning algorithms to train open and accessible language models on this task. When compared with the vanilla supervised fine-tuning approach, these methods consistently reduce lose rates on both common and uncommonsense abductive reasoning judged by human evaluators.

==> 0_abstract_OLD.tex <==
\begin{abstract}
\jena{A key requirement for accurately modeling dynamics of events is commonsense reasoning, which has, thus far, focused on predicting what is most likely. We introduce the task (?) of UNcommonsense Reasoning to explore the \textbf{un}usual, \textbf{un}expected, and \textbf{un}likely (yet possible!) situations. In this setting, given a piece of context an unexpected outcome, a model is tasked to reason abductively by generating a natural language explanation that makes the unexpected outcome more likely in the context. To do this, we curate and release a new English language corpus, called \textbf{Uncommonsense}. We also propose a new on-policy imitation learning called X that improves the performance of open and accessible language models on both common, but especially uncommonsense, abductive reasoning. Moreover, we characterize the differences between human and model performance, and show that machine-human collaboration results in highest-quality explanations.} \jena{suggestion. it compacts the first potion into a first sentence, jumping into the "uncommonsense reasoning" much earlier in the abstract. Then the corpus and the methods are introduced right away.} 
%
Accurately modeling the dynamics of events by performing \emph{commonsense reasoning} is a key requirement of useful language technologies.
%   - However, a key ability human language users have is to reason about uncommon or unusual situations, by applying both commonsense knowledge and counterfactual reasoning.
%   - Our systems should be able to reason about these unusual situations, instead of relying on normative assumptions that may be embedded in our systems from only evaluating them on instances of common scenarios. Need to be flexible to violations of commonsense
% Broadly accessible systems must be able to reason about both common knowledge and its exceptions, as exposed through unusual, unexpected, and implausible situations.
%   - Most work on commonsense reasoning has focused on how well models can represent information that is generally considered common ground, and how well they can use this common-ground information in downstream tasks, such as reasoning about particular events that occur or answering questions about what's happening in an image.
However, most existing evaluations of commonsense focus on predicting what is most likely, e.g., selecting the most plausible ending to a story. 
Less attention has been paid to 
% unusual \fb{it's okay to skip unusual, it's getting too long}, unexpected, and 
implausible (yet possible!) situations.
% \jena{doesn't plausible mean possible?}
 % implausible, yet possible, events.
%   - To directly target a system's ability to reason about unusual situations, we study a problem of abductive reasoning, where given some context and an unexpected outcome, our system is tasked with generating a natural language explanation that adds information that makes the unexpected outcome much more likely in the context.
% We focus on abductive reasoning about uncommon situations, where,
We curate and release an new English-language corpus, called \textbf{UNcommonsense}. %-- including contexts paired with unexpected outcomes and abductive explanations.
In our \emph{uncommonsense reasoning} setup, given a piece of context and an \textbf{un}expected outcome, a model is tasked with generating an additive \fb{informative?} natural language explanation that makes the unexpected outcome more likely in the context, e.g., \jack{punchy example?}
% including contexts paired with unexpected outcomes and abductive explanations.
%   - As there are no existing datasets specifically studying unusual outcomes for abductive reasoning, we curate and release two new datasets, including both unexpected outcomes and abductive explanations written by humans, models, and a combination
% To this end, we curate and release an English-language corpus -- \textbf{UNcommonsense} -- including contexts paired with unexpected outcomes and abductive explanations.
%   - We investigate the existing gap between human and model performance and we find it is nuanced; We find that the most powerful language models available have decent performance on this task, but as the likelihood of outcomes decrease, these models still become worse at explaining these situations. We also find that while the models generally provide more details in their explanations, human-written explanations are generally more creative, and the best human explainers provide much higher quality explanations than the best models. 
We characterize the differences % investigate the existing gap
between human and model \fb{not sure, but do we care about model here refering to LLM and not any model?} performance on our task
%, characterize nuanced differences in explanation quality, \jack{differences between what?} 
and show that model-enhanced human-written explanations \jack{is there a less jargon way to say, e.g., ``machine-human collaboration results in the highest-quality explanations?"} combine the benefits of both. 
% \wz{Inspired by the nuanced gap, the best way to collect high-quality explanation is by human-model collaboration something?}
%   - To address this specific abductive reasoning problem, we experiment with training small, open-source models to produce high-quality explanations, through a new learning method that we propose
%   - We evaluate our models not only on our uncommonsense abductive reasoning task, but also on existing abductive commonsense tasks, and find that our learning method significantly improves the performance of these smaller and more accessible models when compared with supervised learning both for common, and especially for uncommon scenarios
Finally, we propose a \as{we explore on-policy imitation learning algorithms} new on-policy imitation learning method that significantly \as{add concrete numbers here for plausibility?} improves the performance of open and accessible language models on both common, but especially uncommonsense, abductive reasoning.
\as{make the method contributions more obvious}
% \wz{would be nice to mention about how we use expert feedback (we are kinda the first to do on-policy learning in the era of LLMs).  I think we could entirely remove the phrase imitation learning but instead use the phrase expert feedback.}
% \as{personally I worry a bit that ``expert feedback'' implies human-given feedback}
% \fb{adding some numbers in terms of amount of improvements would be nice too}


% Abductive reasoning has been extensively studied in natural language processing (NLP).
% Given a context and an outcome, abductive reasoning aims to produce an explanation that bridges the information gap between the context and the outcome.
% Existing benchmarks often focus their evaluation on the outcomes that become obvious immediately after seeing the contexts.
% However, outcomes can be unexpected, in which new information is necessary to make sense of such outcomes.
% The ability to understand and make inferences for these less common scenarios is essential for building robust and generalizable NLP systems.
% This paper therefore proposes to evaluate abductive reasoning for both common and uncommon events.
% To this end, we collect two datasets specifically designed for abdutive reasoning for uncommon events, where a gap still exist between best humans and best language models including GPT-4.

% A standard method for abductive reasoning is to collect offline expert demonstrations and perform standard supervised learning on such data. However, this approach is prone to mistakes due to distributional shifts. Inspired by recent advances in imitation learning and learning from expert feedback, we propose an on-policy learning method that corrects mistakes during training. Recognizing that interactive experts can be costly or unavailable, we also introduce an offline variant for mistake correction.
% Our proposed methods have demonstrated significant improvements on both the two newly introduced datasets for uncommon events and two existing datasets for common events.
\end{abstract}


% Paper story (Alane)
% Motivation: 
%
% What we do:


==> tables/gpt4-breakdown-by-likelihood.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{lcc}
\toprule
$l$ & \social &\story \\ \midrule
3 & 82.1 (57.1) & 94.2 (39.0) \\
2 & 85.8 (66.5) & 94.0 (43.0) \\
1 & 88.3 (71.9) & 96.6 (49.8) \\
\bottomrule
\end{tabular}
\caption{Win rates of \llmhuman versus \llm, broken down by the likelihoods $l$ of outcomes. We %additionally 
report win rates excluding ties in the parentheses. Greater likelihoods are associated with more likely outcomes.}
\label{tab:gpt4-breakdown-by-likelihood}
\end{table}

==> tables/human_gpt4_analysis.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lcc}
\toprule
      & Unique tokens & \% at 99-percentile \\ \midrule
GPT4 & 10313         & 2.2                 \\
Crowd  & 10039         & 4.0                \\
\bottomrule
\end{tabular}
\caption{Diversity analysis on crowd-written explanations and GPT4-generated explanations. We compute the number of unique tokens and how many unique tokens account for 99\% occurrences.}
\label{tab:human-gpt4-analysis}
\end{table}

==> tables/human_preference.tex <==
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lcc}
% \toprule
%              & \story & \social \\ \midrule
% Crowd        & 17.4\% &30.93\%\\
% GPT4        & \textbf{65.3\%} &\textbf{49.24\%}\\
% Equally {\color{green}Good} & 14.9\% &16.90\%\\
% Equally {\color{red}Bad}  & 2.4\%  &2.93\%\\
% \bottomrule
% \end{tabular}
% \caption{Human preference on crowd-written explanations vs. GPT4-generated explanations.}
% \label{tab:human-preference}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{lcc}
% \toprule
%          & \social &\story \\ \midrule
% Human       & 54 (23) & 52 (14) \\
% Human-GPT4 & 74 (47) & 73 (34) \\
% GPT4-GPT4 & 89 (36) & 80 (27) \\
% \bottomrule
% \end{tabular}
% \caption{Comparison between the win rates of different human-written explanations against model-generated explanations from GPT4. We additionally report win rates excluding ties in the parentheses. Greater likelihoods associate with more likely outcomes.}
% \label{tab:win-rate-human-gpt4}
% \end{table}

\begin{table*}[]
\centering
\footnotesize
\begin{tabular}{lcccccc}
\toprule
     & \multicolumn{3}{c}{\story} & \multicolumn{3}{c}{\social} \\ 
     & \emph{Crowd}     & \emph{C+LLM}     & \emph{LLM$^2$}    & \emph{Crowd}     & \emph{C+LLM}     & \emph{LLM$^2$}      \\ \midrule
Win  & 14 | 12        & 34 | 77            & 27 | 35          & 23 | 28       & 47 | 94             & 36 | 72           \\
Equally good  & 32 | \phantom{0}2        & 35 | \phantom{0}6            & 49 | 59          & 29 | \phantom{0}2       & 27 | \phantom{0}1            & 51 | 24         \\
Equally bad  & \phantom{0}6 | \phantom{0}0       & \phantom{0}4 | \phantom{0}0            & \phantom{0}4 | \phantom{0}0          & \phantom{0}2 | \phantom{0}0       & \phantom{0}0 | \phantom{0}0            & \phantom{0}2 | \phantom{0}0         \\ 
Lose & 48 | 86       & 27 | 17            & 20 | \phantom{0}6          & 46 | 70       & 26 | \phantom{0}5            & 11 | \phantom{0}4           \\
\bottomrule
\end{tabular}
\caption{Preference judgments given by Crowdworkers | GPT-4 comparing explanations from \emph{LLM} with explanations from \emph{Crowd}, \emph{C+LLM}, and \emph{LLM$^2$}.}
\label{tab:win-rate-human-gpt4}
\end{table*}

==> tables/win-rate-human-gpt4.tex <==
% \begin{table}[t]
% \centering
% \begin{tabular}{lcc}
% \toprule
%          & \social &\story \\ \midrule
% Human       & 46.87 & 31.40 \\
% % Authors      & 82.00 & 72.27 \\
% Human-GPT4 & 84.80 & 93.70 \\
% \bottomrule
% \end{tabular}
% \caption{Comparison between the win rates of different human-written explanations against model-generated explanations from GPT4.}
% \label{tab:win-rate-human-gpt4}
% \end{table}
